3D attention mechanism for fine-grained classification of table tennis strokes using a Twin Spatio-Temporal Convolutional Neural Networks

The paper addresses the problem of recognition of actions in video with low inter-class variability such as Table Tennis strokes. Two stream, "twin" convolutional neural networks are used with 3D convolutions both on RGB data and optical flow. Actions are recognized by classification of temporal windows. We introduce 3D attention modules and examine their impact on classification efficiency. In the context of the study of sportsmen performances, a corpus of the particular actions of table tennis strokes is considered. The use of attention blocks in the network speeds up the training step and improves the classification scores up to 5% with our twin model. We visualize the impact on the obtained features and notice correlation between attention and player movements and position. Score comparison of state-of-the-art action classification method and proposed approach with attentional blocks is performed on the corpus. Proposed model with attention blocks outperforms previous model without them and our baseline.

==> answer.tex <==
\newpage
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.07} % Renaud

\section*{Author's Response to reviewers}

We would like to thank the reviewers for their comments for improving our work. In this section we present the modifications made to the paper accordingly to the reviews and answer each point raised by the reviewers.
\\

\textbf{Associate Editor:}

\begin{itemize}

    \item \emph{``
    This paper was reviewed by four experts in the field. The paper received a mixed review. The reviewers raised their concerns on lack of novelty, unconvincing experiment, and the presentation of this paper, While the paper clearly has merit, the decision is not to recommend acceptance. The authors are encouraged to consider the reviewers' comments when revising the paper for resubmission. 
    ''}
    
     Thank you for your comments. We have better highlighted our motivations and the novelty of the proposed method in section~\ref{sec:intro}. We have also conducted further experiments to compare our work in the new subsection~\ref{subsection:classificationperformances}~Classification performances, and modified the title to ``\ArticleTitle'' as advised by one reviewer. Each point raised by each reviewer are answered below.
    \\
\end{itemize}

\textbf{Reviewer 1:}

\begin{itemize}
    \item \emph{``
    This sentence about 3D CNNs: ``two spatial convolutions and one temporal convolution'' may be misleading as it reads as 3 separate convolutions.
    ''}

    Thank you for pointing this out to us. We have replaced it in section~\ref{sec:intro} by ``In this paper, we propose [...]''.
    
    \item \emph{``
    The novelty is easy to grasp from the final para of the intro. The 3D attention block architecture design is interesting in general, and gives good result on this specific dataset and task. It would be nice to have more results of this attention design on standard benchmarking datasets for action recognition, where one can better compare with a larger pool of related works.
    ''}
    
    Thank you for your remarks. Unfortunately, due to lack of time we are not able to present results here on generic action dataset such as UCF-101~\cite{Dataset:UCF101}. However, our context is fine grained action recognition, which has some differences with (coarse grained) action recognition: as shown very recently in the works of~\cite{Dataset:Gym}, there are evidences that a method performing well on a general (coarse grained) action dataset does not necessarily imply a good performance on a fine-grained action dataset. The reason is that general dataset target coarse-grained action understanding  (playing soccer, running,  etc.),  and the background  context  often  provides  distinguishing signals, rather than the actions themselves. On these general dataset, sparse sampling is often sufficient for action recognition, illustrating the fact that temporal information is not the most discriminant one. Contrary to that, in methods developed for fine-grained action dataset, the optical flow (and hence temporal information) plays a major role, and is essential in our proposed method using Twin CNN (RGB+Optical Flow).\\
    We however provide the comparison with the I3D model~\cite{NN:I3DCarreira} applied on our dataset in subsection~\ref{subsection:convergence}: ``We compared our results [...]'' and in the new subsection~\ref{subsection:classificationperformances}~Classification performances: ``Our implemented attention blocks have shown [...]''.\\
    We also make our implementation available to the scientific community\footnote{\url{https://github.com/P-eMartin/crisp}} and are also working on sharing our dataset \texttt{TTStroke21}, with sub-samples already available through the MediaEval workshop\footnote{\url{https://multimediaeval.github.io/editions/2020/tasks/sportsvideo/}}.
    
    \item \emph{``
    There are more works to consider, e.g. videolstm,
    attentional pooling, lsta, video action transformer are all
    attention based and successfully applied to action
    recognition. Since ``movement (optical flow) plays the
    discriminating role'' in your model design, you might be
    interested also in this work ``Paying More Attention to
    Attention, ICLR17''
    ''}
    
     Thank you for these suggestions. Attention models in NNs are now very much popular. We have quite a large experience with attention-based pooling~\cite{Attention::saliency} which we have already referenced in~\ref{subsection:2DAtt}. Now we have shortly analysed referenced ``Paying More Attention to Attention, ICLR17'', we also know this paper and we do agree that there is some similarity in our approaches, see~\ref{subsection:2DAtt} ``Other works such as~\cite{Attention::Transfer} propose ``Teacher-student'' networks where [...]''.
    
    \item \emph{``
    Since ``Two-Stream, NIPS15'' is well known, authors might want to add a few sentence to highlight the main difference
    to their twin model.
    ''}

     Thank you for this remark. Indeed, the main differences from other well known networks~\cite{NN:SimonyanTwoStream, NN:TwoStreamFusion, NN:3dObjectPoposal} lie in the symmetries of our network, the type of input being 4D data (horizontal, vertical , temporal and channel) and the final fusion at the end of our two branches with a bi-linear layer. We now highlight them in section~\ref{section:architecture}: ``The difference from others Two stream networks [...]''.
    
    \item \emph{``
    Given the large increase in parameters (table 1), one might wonder if this might need to consume more labeled data to train robustly. But the ttstroke-21 dataset seems rather limited in scale, could that be discussed in the paper?
    ''}

    Thank you for your interest. The attentions blocks applied to our networks, even if they greatly increase the number of parameters, seems to not lead to over-fitting. However, after have incorporated the comparison with the I3D model~\cite{NN:I3DCarreira}, which is far more deeper and has much more parameters to learn, we can notice that their model leads to over-fitting on our dataset.\\
    We now discuss this matter in section~\ref{subsection:convergence}: ``We can notice the gap between [...]''.

    \item \emph{``
    As a side note, i remember some twitter msg on concurrent
    work called TTNet that authors might be interested
    ''}
    
     Thank you for this information. We have been already in contact with the authors of~\cite{TT:TTNet} as their works are indeed interesting and close to ours. Even if their goal is currently not to do strokes detection and classification and they are mainly focusing on real-time applications, we have now referenced the paper in section~\ref{sec:intro}: ``In~\cite{TT:TTNet}, the authors [...]''.
    \\
\end{itemize}

\textbf{Reviewer 2:}

\begin{itemize}

    \item \emph{``
    [...] However, lack of motivation and comparative study are my major concerns.
    ''}
    
    Thank you for this remark. We have expanded our motivation on table tennis and comparative study in section~\ref{sec:intro}: ``Table tennis strokes are most [...]''
    
    \item \emph{``
    It is clear that a 3D convolutional neural network would
    help with the information discovery and leads to better
    detection results. However, it is not clear why the network
    structure was as designed in the paper and why the transfer
    functions were selected. 
    ''}
    
    Thank you for pointing this out to us. The previous architecture was introduced in our previous work~\cite{PeMTAP} where we stress our choice of architecture. In this paper focus on attention mechanism that are inspired from the work carried in 2D~\cite{Attention::RANImageClassification}. We have clarify this matter in section~\ref{section:architecture}: ``Its architecture without attention blocks [...]''.
    
    \item \emph{``
    In the experiment section, the reported results include
    the numbers related to the proposed method only, but no
    comparison with the state-of-the-art in the literature,
    which makes the reader very difficult to identify the
    advancement of the proposed approach.
    ''}
    
    To be able to fit our answers in 2 pages, please see answer to reviewer 1, second point.
    
    \item \emph{``
    Does the title include two full sentences?
    ''}
    
    We have modified the title to one sentence: ``\ArticleTitle''.
    \\
\end{itemize}

\textbf{Reviewer 3:}

\begin{itemize}

    \item \emph{``
    The contents of this paper seem technically reasonable, but its applicability is questionable because the only one data set used in the experiment, the dataset is prepared by the authors. We believe that experiments should be conducted with a lot of data.
    ''}
    
    To be able to fit our answers in 2 pages, please see answer to reviewer 1, second point.
    
    \item \emph{``
    Alternatively, you might make the problem of using table tennis videos more clear and argue that this is a model for solving it.
    ''}
    
    Thank you for this suggestion. We have expanded our motivation on table tennis and clarified our objectives in section~\ref{sec:intro}: ``Table tennis strokes are most [...]'' and ``In this paper, we propose  [...]''
    \\
\end{itemize}


\textbf{Reviewer 4:}

\begin{itemize}

% In summary, the paper lacks comparison with the state of
% the art 3D attension works to justify its contribution.
% It'll help if the authors can justify their
% contributions and provide evidence that their method is new
% and can outperform more advanced methods instead of some
% simple baselines.
% Also, it's not clear why adding optical flow drastically
% decrease the performance. I don't think the current
% submission is ready. I would encourage the
% authors to address the problems for a future submission.

    \item \emph{``
    [1] J. Liu et al., Global Context-Aware Attention LSTM Networks for 3D Action Recognition, CVPR 2017}
    
    \emph{[2] J. Cai et al., 3D RANs: 3D Residual Attention Networks for action recognition, The Visual Computer, 2019}

    \emph{[...] Incorporating 3D attention in action recognition has been studied before. The work lacks experimental comparisons against these approaches.
    ''}
    
    Thank you for these information and pointing this out to us. We have incorporated those works and reference more recent articles in section~\ref{sec:intro}: ``Attention mechanisms for action recognition [...]''. We also analyse current approaches of attention in action recognition in section~\ref{subsection:3DAtt}: ``3D attention blocks have recently [...]''.\\
    Furthermore, to be able to fit our answers in 2 pages, please see also answer to reviewer 1, second point.
    
    \item \emph{``
    A comparison with the authors' published paper [10] is also
    missed, given the fact this paper has a close connection
    with that one. Without such experimental
    evidences, it's impossible to determine the contribution of
    this work.
    ''}
    
    Indeed the contributions were not cleared compared to our previous work. We have incorporated the performances from our last work~\cite{PeICIP} from the model in~\cite{PeCBMI} in the new subsection ~\ref{subsection:classificationperformances}~Classification performances: ``Our implemented attention blocks have shown [...]''.
    
    \item \emph{``
    It does not make sense that optical flow + RGB performs much worse than RGB alone when using attention. The interpretation ``the insufficient size of batch'' provided by this work is not convincing.
    ''}

     Thank you for this remark. Indeed we presented results at $500$ epochs and the convergence was not over yet. The Twin model might be slower to train due to greater number of parameters to train and lower batch-size, but its final performances are greater. We modified our argumentation in section~\ref{subsection:convergence}: ``With other models, [...]'' and also in the new subsection~\ref{subsection:classificationperformances}: ``From the visualization analysis [...]''.
    
    \item \emph{``
    The presentation of this paper needs to be improved. Even the title of this submission is not appropriate.
    ''}
    
    Thank you for your suggestions. We have modified the abstract, we have enriched the content in sections~\ref{sec:intro}, \ref{section:related_works}; modified the subsection~\ref{subsection:convergence} as its related table: table~\ref{table:acc_500} and added a new subsection~\ref{subsection:classificationperformances} as well. Finally, the title has been modified to: ``\ArticleTitle''

\end{itemize}

% Comments to author (Associate Editor)
% =====================================

% This paper was reviewed by four experts in the field. The
% paper received a mixed review. The reviewers raised their
% concerns on lack of novelty, unconvincing experiment, and
% the presentation of this paper, While the paper clearly has
% merit, the decision is not to recommend acceptance. The
% authors are encouraged to consider the reviewers' comments
% when revising the paper for resubmission. 

% Reviewer 1 of ICPR 2020 submission 1647

% Comments to the author
% ======================

% This sentence about 3D CNNs: ``two spatial convolutions and
% one temporal convolution'' may be misleading as it reads as
% 3 separate convolutions.

% The description of ``The complexity of this data'' is useful
% to get a grasp of difficulty on this novel and non standard
% type of data, showing that it needs finegrained capability
% of differentiating subtile differences in the appearance of
% fast movements.

% The novelty is easy to grasp from the final para of the
% intro. The 3D attention block architecture design is
% interesting in general, and gives good result on this
% specific dataset and task. It would be nice to have more
% results of this attention design on standard benchmarking
% datasets for action recognition, where one can better
% compare with a larger pool of related works.  

% There are more works to consider, e.g. videolstm,
% attentional pooling, lsta, video action transformer are all
% attention based and successfully applied to action
% recognition. Since ``movement (optical flow) plays the
% discriminating role'' in your model design, you might be
% interested also in this work ``Paying More Attention to
% Attention, ICLR17''

% Since ``Two-Stream, NIPS15'' is well known, authors might
% want to add a few sentence to highlight the main difference
% to their twin model.

% Given the large increase in parameters (table 1), one might
% wonder if this might need to consume more labeled data to
% train robustly. But the ttstroke-21 dataset seems rather
% limited in scale, could that be discussed in the paper?

% If these are taken into account in the final paper version
% then i strongly believe the paper should be accepted to
% ICPR.

% As a side note, i remember some twitter msg on concurrent
% work called TTNet that authors might be interested
	



% Reviewer 2 of ICPR 2020 submission 1647

% Comments to the author
% ======================

% This paper proposed a video attention detection method
% using the spatial-temporal features of RGB pixels and
% optical flow. The described approach seems reasonable and
% reported results look good. However, lack of motivation and
% comparative study are my major concerns. 

% - It is clear that a 3D convolutional neural network would
% help with the information discovery and leads to better
% detection results. However, it is not clear why the network
% structure was as designed in the paper and why the transfer
% functions were selected. 

% - In the experiment section, the reported results include
% the numbers related to the proposed method only, but no
% comparison with the state-of-the-art in the literature,
% which makes the reader very difficult to identify the
% advancement of the proposed approach.

% - Does the title include two full sentences?


% Reviewer 3 of ICPR 2020 submission 1647

% Comments to the author
% ======================

% In this paper, a new three-dimensional attentional model is
% proposed and its application to the classification of table
% tennis videos is shown.

% The contents of this paper seem technically reasonable, but
% its applicability is questionable because the only one data
% set used in the experiment, the dataset is prepared by the
% authors. We believe that experiments should be conducted
% with a lot of data. Alternatively, you might make the
% problem of using table tennis videos more clear and argue
% that this is a model for solving it.


% Reviewer 4 of ICPR 2020 submission 1647

% Comments to the author
% ======================

% The paper propose to use 3D convolution in conjunction with
% 3D attention to improve the performance of action
% recognition.
% In particular, their task is to recognize actions in table
% tennis videos, where they show the 3D attention is able to
% improve the recognition accuracy.

% Pros:
% Recognizing actions of athletes is important and has a
% number of potential applications.
% The idea of combing 3D convolution and 3D attention makes
% sense.

% Cons:
% 1) Incorporating 3D attention in action recognition has
% been studied before. The work lacks experimental
% comparisons against these approaches.
% A comparison with the authors' published paper [10] is also
% missed, given the fact this paper has a close connection
% with that one. Without such experimental
% evidences, it's impossible to determine the contribution of
% this work.
% 2) It does not make sense that optical flow + RGB performs
% much worse than RGB alone when using attention. The
% interpretation ``the insufficient size of batch''
% provided by this work is not convincing.
% 3) The presentation of this paper needs to be improved.
% Even the title of this submission is not appropriate.

% [1] J. Liu et al., Global Context-Aware Attention LSTM
% Networks for 3D Action Recognition, CVPR 2017
% [2] J. Cai et al., 3D RANs: 3D Residual Attention Networks
% for action recognition, The Visual Computer, 2019


% In summary, the paper lacks comparison with the state of
% the art 3D attension works to justify its contribution.
% It'll help if the authors can justify their
% contributions and provide evidence that their method is new
% and can outperform more advanced methods instead of some
% simple baselines.
% Also, it's not clear why adding optical flow drastically
% decrease the performance. I don't think the current
% submission is ready. I would encourage the
% authors to address the problems for a future submission.
